The Dynamic Evolution of Solar Wind Streams Following Interchange Reconnection

Interchange reconnection is thought to play an important role in determining the dynamics and material composition of the slow solar wind that originates from near coronal hole boundaries. To explore the implications of this process we simulate the dynamic evolution of a solar wind stream along a newly-opened magnetic flux tube. The initial condition is composed of a piecewise continuous dynamic equilibrium in which the regions above and below the reconnection site are extracted from steady-state solutions along open and closed field lines. The initial discontinuity at the reconnection site is highly unstable and evolves as a Riemann problem, decomposing into an outward-propagating shock and inward-propagating rarefaction that eventually develop into a classic N-wave configuration. This configuration ultimately propagates into the heliosphere as a coherent structure and the entire system eventually settles to a quasi-steady wind solution. In addition to simulating the fluid evolution we also calculate the time-dependent non-equilibrium ionization of oxygen in real time in order to construct in situ diagnostics of the conditions near the reconnection site. This idealized description of the plasma dynamics along a newly-opened magnetic field line provides a baseline for predicting and interpreting the implications of interchange reconnection for the slow solar wind. Notably, the density and velocity within the expanding N-wave are generally enhanced over the ambient wind, as is the O7+/O6+ ionization ratio, which exhibits a discontinuity across the reconnection site that is transported by the flow and arrives later than the propagating N-wave.

==> The Dynamic Evolution of Solar Wind Streams Following Interchange Reconnection/journal_defs.tex <==
\newcommand\aj{\rmfamily AJ}%
          % Astronomical Journal
\newcommand\actaa{\rmfamily Acta Astron.}%
  % Acta Astronomica
\newcommand\araa{\rmfamily ARA\&A}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\rmfamily ApJ}%
          % Astrophysical Journal
\newcommand\apjl{\rmfamily ApJ}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\rmfamily ApJS}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\rmfamily Appl.~Opt.}%
          % Applied Optics
\newcommand\apss{\rmfamily Ap\&SS}%
          % Astrophysics and Space Science
\newcommand\aap{\rmfamily A\&A}%
          % Astronomy and Astrophysics
\newcommand\aapr{\rmfamily A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\rmfamily A\&AS}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\rmfamily AZh}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\rmfamily BAAS}%
          % Bulletin of the AAS
\newcommand\caa{\rmfamily Chinese Astron. Astrophys.}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{\rmfamily Chinese J. Astron. Astrophys.}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{\rmfamily Icarus}%
  % Icarus
\newcommand\jcap{\rmfamily J. Cosmology Astropart. Phys.}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{\rmfamily JRASC}%
          % Journal of the RAS of Canada
\newcommand\memras{\rmfamily MmRAS}%
          % Memoirs of the RAS
\newcommand\mnras{\rmfamily MNRAS}%
          % Monthly Notices of the RAS
\newcommand\na{\rmfamily New A}%
  % New Astronomy
\newcommand\nar{\rmfamily New A Rev.}%
  % New Astronomy Review
\newcommand\pra{\rmfamily Phys.~Rev.~A}%
          % Physical Review A: General Physics
\newcommand\prb{\rmfamily Phys.~Rev.~B}%
          % Physical Review B: Solid State
\newcommand\prc{\rmfamily Phys.~Rev.~C}%
          % Physical Review C
\newcommand\prd{\rmfamily Phys.~Rev.~D}%
          % Physical Review D
\newcommand\pre{\rmfamily Phys.~Rev.~E}%
          % Physical Review E
\newcommand\prl{\rmfamily Phys.~Rev.~Lett.}%
          % Physical Review Letters
\newcommand\pasa{\rmfamily PASA}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{\rmfamily PASP}%
          % Publications of the ASP
\newcommand\pasj{\rmfamily PASJ}%
          % Publications of the ASJ
\newcommand\qjras{\rmfamily QJRAS}%
          % Quarterly Journal of the RAS
\newcommand\rmfamilyxaa{\rmfamily Rev. Mexicana Astron. Astrofis.}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{\rmfamily S\&T}%
          % Sky and Telescope
\newcommand\solphys{\rmfamily Sol.~Phys.}%
          % Solar Physics
\newcommand\sovast{\rmfamily Soviet~Ast.}%
          % Soviet Astronomy
\newcommand\ssr{\rmfamily Space~Sci.~Rev.}%
          % Space Science Reviews
\newcommand\zap{\rmfamily ZAp}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{\rmfamily Nature}%
          % Nature
\newcommand\iaucirc{\rmfamily IAU~Circ.}%
          % IAU Cirulars
\newcommand\aplett{\rmfamily Astrophys.~Lett.}%
          % Astrophysics Letters and Communications
\newcommand\apspr{\rmfamily Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\newcommand\bain{\rmfamily Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\eps{\rmfamily EPS}%
	% Earth, Planets and Space
\newcommand\fcp{\rmfamily Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\newcommand\gca{\rmfamily Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\rmfamily Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\newcommand\jcp{\rmfamily J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\newcommand\jgr{\rmfamily JGR}%
          % Journal of Geophysical Research
\newcommand\jqsrt{\rmfamily J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\rmfamily Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\rmfamily Nucl.~Phys.~A}%
          % Nuclear Physics A
\newcommand\physrep{\rmfamily Phys.~Rep.}%
          % Physics Reports
\newcommand\physscr{\rmfamily Phys.~Scr}%
          % Physica Scripta
\newcommand\planss{\rmfamily Planet.~Space~Sci.}%
          % Planetary Space Science
\newcommand\procspie{\rmfamily Proc.~SPIE}%
          % Proceedings of the SPIE

==> journal_defs.tex <==
\newcommand\aj{\rmfamily AJ}%
          % Astronomical Journal
\newcommand\actaa{\rmfamily Acta Astron.}%
  % Acta Astronomica
\newcommand\araa{\rmfamily ARA\&A}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\rmfamily ApJ}%
          % Astrophysical Journal
\newcommand\apjl{\rmfamily ApJ}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\rmfamily ApJS}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\rmfamily Appl.~Opt.}%
          % Applied Optics
\newcommand\apss{\rmfamily Ap\&SS}%
          % Astrophysics and Space Science
\newcommand\aap{\rmfamily A\&A}%
          % Astronomy and Astrophysics
\newcommand\aapr{\rmfamily A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\rmfamily A\&AS}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\rmfamily AZh}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\rmfamily BAAS}%
          % Bulletin of the AAS
\newcommand\caa{\rmfamily Chinese Astron. Astrophys.}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{\rmfamily Chinese J. Astron. Astrophys.}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{\rmfamily Icarus}%
  % Icarus
\newcommand\jcap{\rmfamily J. Cosmology Astropart. Phys.}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{\rmfamily JRASC}%
          % Journal of the RAS of Canada
\newcommand\memras{\rmfamily MmRAS}%
          % Memoirs of the RAS
\newcommand\mnras{\rmfamily MNRAS}%
          % Monthly Notices of the RAS
\newcommand\na{\rmfamily New A}%
  % New Astronomy
\newcommand\nar{\rmfamily New A Rev.}%
  % New Astronomy Review
\newcommand\pra{\rmfamily Phys.~Rev.~A}%
          % Physical Review A: General Physics
\newcommand\prb{\rmfamily Phys.~Rev.~B}%
          % Physical Review B: Solid State
\newcommand\prc{\rmfamily Phys.~Rev.~C}%
          % Physical Review C
\newcommand\prd{\rmfamily Phys.~Rev.~D}%
          % Physical Review D
\newcommand\pre{\rmfamily Phys.~Rev.~E}%
          % Physical Review E
\newcommand\prl{\rmfamily Phys.~Rev.~Lett.}%
          % Physical Review Letters
\newcommand\pasa{\rmfamily PASA}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{\rmfamily PASP}%
          % Publications of the ASP
\newcommand\pasj{\rmfamily PASJ}%
          % Publications of the ASJ
\newcommand\qjras{\rmfamily QJRAS}%
          % Quarterly Journal of the RAS
\newcommand\rmfamilyxaa{\rmfamily Rev. Mexicana Astron. Astrofis.}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{\rmfamily S\&T}%
          % Sky and Telescope
\newcommand\solphys{\rmfamily Sol.~Phys.}%
          % Solar Physics
\newcommand\sovast{\rmfamily Soviet~Ast.}%
          % Soviet Astronomy
\newcommand\ssr{\rmfamily Space~Sci.~Rev.}%
          % Space Science Reviews
\newcommand\zap{\rmfamily ZAp}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{\rmfamily Nature}%
          % Nature
\newcommand\iaucirc{\rmfamily IAU~Circ.}%
          % IAU Cirulars
\newcommand\aplett{\rmfamily Astrophys.~Lett.}%
          % Astrophysics Letters and Communications
\newcommand\apspr{\rmfamily Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\newcommand\bain{\rmfamily Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\eps{\rmfamily EPS}%
	% Earth, Planets and Space
\newcommand\fcp{\rmfamily Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\newcommand\gca{\rmfamily Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\rmfamily Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\newcommand\jcp{\rmfamily J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\newcommand\jgr{\rmfamily JGR}%
          % Journal of Geophysical Research
\newcommand\jqsrt{\rmfamily J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\rmfamily Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\rmfamily Nucl.~Phys.~A}%
          % Nuclear Physics A
\newcommand\physrep{\rmfamily Phys.~Rep.}%
          % Physics Reports
\newcommand\physscr{\rmfamily Phys.~Scr}%
          % Physica Scripta
\newcommand\planss{\rmfamily Planet.~Space~Sci.}%
          % Planetary Space Science
\newcommand\procspie{\rmfamily Proc.~SPIE}%
          % Proceedings of the SPIE
